Marlin: Knowledge-Driven Analysis of Provenance Graphs for Efficient and Robust Detection of Cyber Attacks

Recent research in both academia and industry has validated the effectiveness of provenance graph-based detection for advanced cyber attack detection and investigation. However, analyzing large-scale provenance graphs often results in substantial overhead. To improve performance, existing detection systems implement various optimization strategies. Yet, as several recent studies suggest, these strategies could lose necessary context information and be vulnerable to evasions. Designing a detection system that is efficient and robust against adversarial attacks is an open problem. We introduce Marlin, which approaches cyber attack detection through real-time provenance graph alignment.By leveraging query graphs embedded with attack knowledge, Marlin can efficiently identify entities and events within provenance graphs, embedding targeted analysis and significantly narrowing the search space. Moreover, we incorporate our graph alignment algorithm into a tag propagation-based schema to eliminate the need for storing and reprocessing raw logs. This design significantly reduces in-memory storage requirements and minimizes data processing overhead. As a result, it enables real-time graph alignment while preserving essential context information, thereby enhancing the robustness of cyber attack detection. Moreover, Marlin allows analysts to customize attack query graphs flexibly to detect extended attacks and provide interpretable detection results. We conduct experimental evaluations on two large-scale public datasets containing 257.42 GB of logs and 12 query graphs of varying sizes, covering multiple attack techniques and scenarios. The results show that Marlin can process 137K events per second while accurately identifying 120 subgraphs with 31 confirmed attacks, along with only 1 false positive, demonstrating its efficiency and accuracy in handling massive data.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Pseudocode_BaselineDB.tex <==
\begin{algorithm}
    \SetAlgoLined
    \KwData{this text}
    \KwResult{how to write algorithm with \LaTeX2e }
  
    initialization\;
    \While{not at end of this document}{
      read current\;
      \eIf{understand}{
        go to next section\;
        current section becomes this one\;
        }{
        go back to the beginning of current section\;
        }
      }
    \caption{How to write algorithms}
\end{algorithm}
%   https://zhuanlan.zhihu.com/p/166418214

==> Pseudocode_CrossHostMerge.tex <==
\begin{algorithm}
    \caption{Cross-host Alert Merge}\label{algo:cross_host_merge}
    \SetAlgoLined
    \KwData{existing tag $T$, new event $E_i$ and corresponding event regular score $S_{Ei}$ and.}
    \KwResult{propagated tag $T'$.}
    $S_P \leftarrow T.S_P \cdot S_{Ei} \cdot \alpha$; \tcp{calculate path regualr score}
    \eIf{$S_{Ei} > S_P$}{
        $T'.S_P \leftarrow S_P$; \tcp{update anomaly score}
        $T'.P$.\textsc{Add}($E_i$); \tcp{add event to anomaly path}
    }{
        $T'.S_P \leftarrow S_{Ei}$; \tcp{update anomaly score}
        $T'.P \leftarrow$ [$E_i$]; \tcp{init new anomaly path}
    }
    \Return{$T'$}\;
\end{algorithm}
%   https://zhuanlan.zhihu.com/p/166418214

==> Pseudocode_InitTag.tex <==
\begin{algorithm}
    \caption{Init Tag}\label{algo:init_tag}
    \SetAlgoLined
    \KwData{technological knowledge graph $TKG$, and seed node $SN$}
    \KwResult{tag $T$.}
    \tcc{create new tag}
    $T \leftarrow new\ (SN, TKG)$\; 
    \tcc{init last aligned node}
    $T.lastAlignedNode \leftarrow SN$\; 
    \tcc{init align status}
    $T.alignStatus \leftarrow new\ TKGStatus(TKG, SN)$\;
    \tcc{init search Graph} 
    $T.searchGraph \leftarrow new\ (TKG)$\; 
    \Return{$T$}\; 
    % \vspace{\baselineskip}
    % \begin{CJK*}{UTF8}{gbsn}
    % % 算法二主要讲解了标签初始化流程:
    % % (1)使用seedNode作为标签初始化时第一次的lastAlignedNode
    % % (2)使用TKG去创建searchTree
    % % (3)使用TKG和seedNode去创建GraphAlignmentStatus.
    % \end{CJK*}
\end{algorithm}
%   https://zhuanlan.zhihu.com/p/166418214

==> Pseudocode_MergeTag.tex <==
\begin{algorithm}
    \caption{Merge Tag}\label{algo:merge_tag}
    \SetAlgoLined
    \KwData{existing Tag $T$ and $T'$.}
    \KwResult{Tag $T$.}
    
    \If{$T.\text{recurringAlert()}$}{
        \Return{null}\;
    }
    $T.\text{mergeTKGStatus}(T')$\;
    \If{$\text{Alignment\_Threshold} \leq \text{TKGStatus.Score}$}{
        \tcc{Trigger Alert}
        \Return{null}\;
    }
    \eIf{$T$.\text{isOnTKG()}}{ 
        $T.\text{lastAlignedNode} \leftarrow T'.\text{lastAlignedNode}$;
    }{
        $T.\text{lastAlignedNode} \leftarrow \text{null}$;
    }
    \Return{$T$}\;
    % \vspace{\baselineskip}
    % \begin{CJK*}{UTF8}{gbsn}
    % % 算法四主要讲解了标签的合并流程:
    % % (1)判断标签T是否已经触发过告警
    % % (2)将标签T和标签T'的TKG对齐状态进行合并,并重新计算anomalyScore
    % % (3)判断合并后的标签是否满足告警的条件
    % % (4)如果标签节点的位置与TKG上的节点对应,lastAlignedNode更新为TKG上的节点,否则置为null;
    % \end{CJK*}
\end{algorithm}
%   https://zhuanlan.zhihu.com/p/166418214

==> Pseudocode_SingleHostMerge.tex <==
\begin{algorithm}
    \caption{Single-host Alert Merge}\label{algo:single_host_merge}
    \SetAlgoLined
    \KwData{tags that trige alert $T$.}
    \KwResult{merged alerts $T'$.}
    $S_P \leftarrow T.S_P \cdot S_{Ei} \cdot \alpha$; \tcp{calculate path regualr score}
    \eIf{$S_{Ei} > S_P$}{
        $T'.S_P \leftarrow S_P$; \tcp{update anomaly score}
        $T'.P$.\textsc{Add}($E_i$); \tcp{add event to anomaly path}
    }{
        $T'.S_P \leftarrow S_{Ei}$; \tcp{update anomaly score}
        $T'.P \leftarrow$ [$E_i$]; \tcp{init new anomaly path}
    }
    \Return{$T'$}\;
\end{algorithm}
%   https://zhuanlan.zhihu.com/p/166418214
